Transforming Medical Regulations into Numbers: Vectorizing a Decade of Medical Device Regulatory Shifts in the USA, EU, and China

Navigating the regulatory frameworks that ensure the safety and efficacy of medical devices can be challenging, especially across different regions. These frameworks often require redundant testing, slowing down the process of getting innovations to patients. This study leverages Natural Language Processing (NLP) to analyze 664 regulations and guidelines from the USA, EU, and China over the past decade, covering over 200 million tokens. We categorize regulations into key phases, such as animal studies, clinical trials, and other testing stages, and use Bidirectional Encoder Representations from Transformers (BERT) to perform Named Entity Recognition (NER), identifying key regulatory terms and entities. By converting these texts into numerical representations and segmenting them by phase, country, and year, we compare jurisdictional requirements and assess their alignment. Additionally, we apply Latent Dirichlet Allocation (LDA) for theme analysis to observe changes in regulatory focus over time, reflecting evolving priorities and challenges. Our analysis reveals notable semantic similarities and differences between countries and phases. For instance, the closest alignment in animal study regulations is between China and the USA, with a mean cosine distance of 0.33. These findings highlight the computational potential in regulatory science, offering valuable insights for researchers, policymakers, and industry professionals.

==> sections/experiments.tex <==
\section{Case Study} \label{Section: case_study}
\subsection{Dataset}
New Jersey (NJ) Turnpike data were used to test the applicability of our model combining Line Graph Convolutional Networks and Kalman filter for Origin-Destination (O-D) prediction. Figure \ref{fig:turnpike_map} shows the simplified map of NJ turnpike. The dataset provides anonymized entrance and exit times of each vehicle, which can be used to calculate aggregated O-D flows. The analysis period is from 6:15 A.M. to 9:45 A.M. with the length of departure interval being 15 minutes. The link flows are calculated at the entrance of each link. We assume that each vehicle has a constant speed $60$ mph to calculate aggregated link flows \cite{ashok1996estimation}. This assumption is unrealistic in real scenarios. However, all we need is a set of consistent O-D and link flows to implement our approach. The issue of whether the constant speed consumption is reasonable is not directly relevant. Since there is only one route for each O-D pair in the NJ Turnpike, the route choice effect is not considered.

\begin{figure*}[hbt]
  \centering
  \includegraphics[width=0.75\textwidth, trim=140 250 130 300,clip]{figures//turnpike_map.pdf}
  \caption{Section of NJ turnpike.}\label{fig:turnpike_map}
\end{figure*}

There are 26 interchanges in this network (Figure \ref{fig:turnpike_map}). The O-D table is thus a $(26 \times 25)$ matrix. We assume that the entrance of each link is equipped with traffic sensors. Since there are two directions, the number of links is $50$. We use aggregated O-D flows and link flows from February 01 to May 31 in 2013, e.g., data in 4 months, to train the neural networks. Then we use O-D flows in June 2013, e.g., data in 1 month, to evaluate our prediction performance.

The platform for implementing our proposed algorithms is a server with 1 GPU (NVIDIA TITAN RTX, 24GB memory). When we trained the FL-GCN, 4 prior intervals, e.g., 1 hour data, were used to predict the next interval O-D flows. Historical O-D and link flows were from the same interval 7 days ago. Real-time and historical link flows were integrated into a $(50 \times 8)$ matrix. We constructed 3 layers of link Graph Convolutional Networks (GCNs) with respective filter size: $(8 \times 100), (100 \times 50)$, and $(50 \times 25)$, 1 layer of line graph transformation with filter size $(25 \times 25)$, and two layers of node GCNs with respective filter size: $(25 \times 50)$, and $(50 \times 25)$. The node adjacency matrix, link adjacency matrix, and incidence matrix were defined according to the topology shown in Figure \ref{fig:turnpike_map}. For the historical O-D demand part, we used Fully Connected Networks (FCNs) and Convolutional Neural Networks (CNNs) to evaluate the spatial correlations. The number of layers in FCN and the number of layers in CNN were both 3. The kernel size of CNN was $(3 \times 3)$. The size of $\mathbf{w_4}$ and the size of $\mathbf{w_5}$ in Equation \eqref{Equation: FL-GCN} were both $(25 \times 25)$.

In Kalman filter, we followed the assumptions in Ashok and Ben-Akiva \cite{ashok2000alternative}. Firstly, the structure of transition matrix remained constant over the whole day. Secondly, a flow between O-D pair $r$ for a period was related only to $r^{th}$ O-D flow of prior intervals, then the transition matrix $\mathbf{f}$ was diagonal. The assignment matrix $\mathbf{a}$ was calculated directly from link counts and O-D flows. In addition, we used deviations from the same interval 7 days ago as state variables \cite{ashok1996estimation}.




\subsection{Numerical Results}
In this section, we use three classical metrics to evaluate the prediction performance: Mean Absolute Error (MAE), Root Mean Square Error (RMSE) and Root Mean Square Error Normalized (RMSN), given by $MAE = \frac{1}{N} \sum_{i=1}^{N} \left| x{^N_i} - \hat{x}{^N_i} \right|$, $RMSE = \sqrt{\frac{1}{N} \sum_{i=1}^{N} \left( x{^N_i} - \hat{x}{^N_i} \right)^2}$, $RMSN = \frac{\sqrt{N \sum_{i} \left( x{^N_i} - \hat{x}{^N_i} \right)^2}}{\sum_{i} x{^N_i}}$, where $N$ is the total number of predicted O-D pairs in June 2013, $\hat{x}{^N_i}$ is the $i^{th}$ predicted O-D flow in the total O-D pairs, and $x{^N_i}$ is the corresponding ground truth. MAE and RMSE are used to measure the absolute difference, and RMSN is used to measure the relative difference.

We have conducted experiments under different prediction steps and  compared the performance of deep neural networks, Kalman filter and the mixing outputs. The models used are shown as follows:

(a). Historical: we use historical data in the same interval 7 days ago as the predicted flows.

(b). Kalman filter: deviation based Kalman filter shown in the methodology section.

(c). FL-GCN-FCN: this approach is FL-GCN without node convolution, and FCN is used to represent the evolution from historical O-D flows to predicted O-D flows.

(d). FL-GCN-CNN: this approach is FL-GCN without node convolution. CNN is used instead to denote the evolution from historical O-D flows to predicted O-D flows.

(e). LGCN-NGCN: this approach is FL-GCN with node convolution, where LGCN denotes the link graph convolution and NGCN represents the node graph convolution. In this approach, we use CNN to represent the evolution from historical O-D flows to predicted O-D flows.

(f). Mixing LGCN-NGCN: combining LGCN-NGCN with Kalman filter, and the parameter $\lambda$ is $0.8$.

(g). Mixing FL-GCN: combining FL-GCN-CNN with Kalman filter, and the parameter $\lambda$ is $0.8$.
 
The results in Table \ref{table:average_results} show that the mixing FL-GCN yields the best performance under different prediction steps. We first compare the performance between deep neural networks and Kalman filter. The results show that the errors in FL-GCN-FCN, FL-GCN-CNN, and LGCN-NGCN are smaller than those in Kalman filter and historical data, which indicate that deep neural networks are effective in recognizing dynamic spatial-temporal O-D patterns. The performance of deep neural networks becomes worse as we increase the prediction step.
 
\begin{table}[hbt]
  \begin{center}
  \caption{Prediction comparison among different models.}\label{table:average_results}
    \begin{tabular}{lllllll}
    \toprule
    Model                             & MAE           & RMSE           & RMSN                                              \\
    \midrule
     (a) 1-Step Predicted                                                                                                  \\
    Historical                        & 3.942         & 8.445          & 0.610                                             \\
    Kalman filter                     & 4.019         & 9.383          & 0.678                                             \\
    FL-GCN-FCN                        & 3.714         & 7.872          & 0.569                                             \\
    FL-GCN-CNN                        & 3.605         & 7.532          & 0.544                                             \\
    LGCN-NGCN                          & 3.607         & 7.557          & 0.546                                             \\
    Mixing LGCN-NGCN              & 3.594         & 7.486          & 0.541                                             \\
    Mixing FL-GCN                  & \textbf{3.585}         & \textbf{7.440}          & \textbf{0.537}                  \\
    \midrule
     (b) 2-Step Predicted \\
    Historical                        & 3.987         & 8.498         & 0.607                                              \\
    Kalman filter                     & 4.052         & 9.378         & 0.670                                              \\
    FL-GCN-FCN                        & 3.778         & 7.956         & 0.568                                              \\
    FL-GCN-CNN                        & 3.681         & 7.653         & 0.547                                              \\
    LGCN-NGCN                         & 3.684         & 7.663         & 0.547                                              \\    
    Mixing LGCN-NGCN               & 3.668        & 7.598         & 0.543                                               \\
    Mixing FL-GCN                 & \textbf{3.649}         & \textbf{7.557}         & \textbf{0.540}                   \\    
    \midrule
     (c) 3-Step Predicted \\
    Historical                        & 4.027         & 8.553         & 0.607                                              \\
    Kalman filter                     & 4.088         & 9.412         & 0.669                                              \\
    FL-GCN-FCN                        & 3.780         & 8.014         & 0.569                                              \\
    FL-GCN-CNN                        & 3.694         & 7.747         & 0.550                                              \\
    LGCN-NGCN                         & 3.743         & 7.820         & 0.555                                              \\    
    Mixing LGCN-NGCN              & 3.702         & 7.683         & 0.546                                              \\
    Mixing FL-GCN                  & \textbf{3.670}         & \textbf{7.642}         & \textbf{0.543}                   \\    
    \bottomrule
    \end{tabular}
    \end{center}
\end{table}

 We then randomly choose several O-D pairs to show the temporal prediction performance. The analysis period is the peak hour from 6:15 A.M. to 9:45 A.M. in June 2013. Figure \ref{fig:results_two_three_step} shows the results in one step, two step and three step predictions respectively. FL-GCN with CNN is used in these cases to yield better performance. From the comparison, we can see that FL-GCN can recognize the temporal patterns better than Kalman filter.
 
\begin{figure}[!ht]
  \centering
  \begin{subfigure}[b]{1.0\textwidth}
  \centering
  \includegraphics[width=0.64\textwidth, trim=60 110 60 140,clip]{figures//step_1.pdf}
  \caption{One step predicted}
  \label{fig:one_step_high_flow}
  \end{subfigure}
  \hfill
  
  \begin{subfigure}[b]{1.0\textwidth}
  \centering
  \includegraphics[width=0.64\textwidth, trim=60 110 60 140,clip]{figures//step_2.pdf}
  \caption{Two step predicted}
  \label{fig:two_step_high_flow}
  \end{subfigure}
  \hfill
  
  \begin{subfigure}[b]{1.0\textwidth}
  \centering
  \includegraphics[width=0.64\textwidth, trim=60 110 60 140,clip]{figures//step_3.pdf}
  \caption{Three step predicted}
  \label{fig:three_step_high_flow}
  \end{subfigure}
  
  
  \caption{Model comparison under different prediction steps.} \label{fig:results_two_three_step}
\end{figure}

 Then we compare the performance using different neural network structures. The results in Table \ref{table:average_results} show that prediction errors in FL-GCN with CNN are smaller than those in FL-GCN with FCN, which indicates that adding CNN to recognize historical O-D correlations can improve prediction performance. The errors in LGCN-NGCN is almost the same with those in FL-GCN-CNN, which shows that adding node graph convolution is not necessary in flow information aggregation. FL-GCN with CNN yields the best performance compared with other models.
 
In addition, errors in mixing LGCN-NGCN are smaller than those in LGCN-NGCN, and errors in mixing FL-GCN are smaller than those in FL-GCN-CNN. The results show that adding appropriate Kalman filter into deep neural networks can improve prediction performance. Mixing FL-GCN is still better than mixing LGCN-NGCN due to better performance in FL-GCN with CNN.

In Table \ref{table:average_results}, the overall performance using different models are evaluated. The predictions of historical data are not much different from the performance of neural networks due to little variability in O-D flows between historical data and true values \cite{ashok1996estimation}. However, historical data cannot incorporate dynamic information, e.g., link flow variation 15 minutes ago, into predicted demands. In FL-GCN, more comprehensive data, i.e., $4$ prior intervals and historical O-D flows, are incorporated into neural networks.

Furthermore, the performance comparison with poor historical information, i.e., historical O-D flows are much different from true O-D flows, is shown in Table \ref{table:high_flows_poor_historical}. When the gap between historical O-D flow and true value is more than $100$ veh / $15 \min$, the O-D demand in that interval would be considered as the pair with poor historical information. The prediction comparison is under high flow level in Table \ref{table:high_flows_poor_historical}. The results show that all neural networks are significantly superior to historical data, especially the FL-GCN with CNN, when the poor historical values are used under the high flow level \cite{ashok1996estimation}.

\begin{table*}[!ht]
  \begin{center}
      \caption{Prediction comparison with poor historical information.}\label{table:high_flows_poor_historical}
    \begin{tabular}{ccccccc}
    
    \hline
    
    \multirow{2}*{Model}              &\multicolumn{3}{c}{Flows $\geq$ 100 [veh / $15 \min$] }                &\multicolumn{3}{c}{Flows $\geq$ 150 [veh / $15 \min$]} \\
    \cline{2-4}
    \cline{5-7}
                    & MAE   & RMSE   & RMSN         & MAE  & RMSE  & RMSN \\
    \hline
    (a) 1-Step Predicted    \\
    Historical      &143.685 &149.679 &0.799        &155.349 &161.396 &0.769 \\
    FL-GCN-FCN      &123.92  &132.357 &0.707        &130.634 &140.350 &0.668 \\
    FL-GCN-CNN      &113.868 &124.660 &0.666        &119.642 &131.784 &0.628 \\
    LGCN-NGCN       &122.085 &129.330 &0.691        &130.579 &138.069 &0.658 \\
    \hline
    (b) 2-Step Predicted \\
    Historical      &142.0     &147.494 &0.799        &153.555 &159.122 &0.767 \\
    FL-GCN-FCN      &114.090 &127.426 &0.690        &122.529 &136.673 &0.659 \\
    FL-GCN-CNN      &118.272 &126.936 &0.688        &125.888 &135.450 &0.653 \\
    LGCN-NGCN       &122.787 &129.427 &0.701        &133.299 &139.845 &0.674 \\
    \hline
    (c) 3-Step Predicted \\
    Historical      &140.197 &145.258 &0.799        &151.807 &156.967 &0.766 \\
    FL-GCN-FCN      &123.464 &131.827 &0.725        &131.247 &140.627 &0.686 \\
    FL-GCN-CNN      &117.356 &125.849 &0.692        &123.073 &132.894 &0.648 \\
    LGCN-NGCN       &121.617 &130.743 &0.719        &131.238 &141.056 &0.688 \\
    \hline
     \end{tabular}
     \end{center}
\end{table*}

\subsection{Analysis of the mixing weight}
In this section, the effect of mixing weight on prediction performance is analyzed. The results in Table \ref{table:high_flows} show the performance when flows are less than and more than $100$ veh / $15 \min$. Kalman filter yields better performance in the high flow level, especially when we use $RMSE$ and $RMSN$ as metrics. In Kalman filter, the predicted O-D flows are obtained by the summation of deviations and historical O-D flows. The pattern of O-D pair with higher flow is more significant than that with lower flow. Historical O-D flows have greater impact on the final prediction when the flow is high.

\begin{table*}[hbt]
  \begin{center}
      \caption{Prediction comparison under different flow levels.}\label{table:high_flows}
    \begin{tabular}{lccccccc}
    
    \hline
    
    \multirow{2}*{Model}              &\multicolumn{3}{c}{Flows $<$ 100 [veh / $15 \min$] }                &\multicolumn{3}{c}{Flows $\geq$ 100 [veh / $15 \min$]} \\
    \cline{2-4}
    \cline{5-7}
                                      & MAE           & RMSE           & RMSN           & MAE           & RMSE           & RMSN       \\
    \hline
    (a) 1-Step Predicted                                                                                                              \\
    Historical                        & 3.557         & 6.628          & 0.593          & 24.582        & 39.222 &0.250                       \\
    Kalman filter                     & 3.671         & 8.298          & 0.742          & 22.664        &33.395 &0.213                       \\
    FL-GCN-FCN                        & 3.348         & 6.219          & 0.556          & 23.262        &36.181 &0.230                 \\
    FL-GCN-CNN                        & 3.263         & 6.005          & 0.537          & 21.934        &34.117 &0.217                 \\
    LGCN-NGCN                         & 3.257         & 5.964          & 0.534          & 22.364        &34.793 &0.222     \\
    Mixing LGCN-NGCN               & 3.249         & 5.966          & 0.534          & 22.080        &33.926 &0.216       \\
    Mixing FL-GCN                   & 3.247         & 5.979          & 0.535          & 21.650        &33.258 &0.212                \\
    \hline
    (b) 2-Step Predicted \\
    Historical                        & 3.592         & 6.675          & 0.590          & 24.685        &39.040 &0.251              \\
    Kalman filter                     & 3.697         & 8.280          & 0.733          & 22.735        &33.246 &0.213               \\
    FL-GCN-FCN                        & 3.421         & 6.419          & 0.568          & 22.510        &34.980 &0.225                 \\
    FL-GCN-CNN                        & 3.332         & 6.088          & 0.538          & 21.994        &34.460 &0.221                 \\
    LGCN-NGCN                         & 3.326         & 6.041          & 0.534          & 22.502        &35.008 &0.225     \\
    Mixing LGCN-NGCN               & 3.315         & 6.051          & 0.535          & 22.232 &34.148 &0.219       \\
    Mixing FL-GCN                  & 3.304         & 6.057          & 0.536          & 21.740 &33.594 &0.216                \\
    \hline
    (c) 3-Step Predicted \\
    Historical                        & 3.625         & 6.722          & 0.591          & 24.803  &38.988  &0.253              \\
    Kalman filter                     & 3.724         & 8.296          & 0.729          & 22.900 &33.333 &0.216               \\
    FL-GCN-FCN                        & 3.394         & 6.280          & 0.552          & 23.729 &36.693 &0.238                 \\
    FL-GCN-CNN                        & 3.328         & 6.115          & 0.538          & 22.588 &35.073 &0.227                 \\
    LGCN-NGCN                         & 3.371         & 6.133          & 0.539          & 22.963 &35.755 &0.232     \\
    Mixing LGCN-NGCN               & 3.311         & 6.088          & 0.535          & 22.245 &34.096 &0.221       \\
    Mixing FL-GCN                  & 3.338         & 6.079          & 0.534          & 22.539 &34.652 &0.225                \\
    \hline
    \end{tabular}
    \end{center}
\end{table*}

The results in Table \ref{table:average_results} show that deep neural networks provide better performance than Kalman filter. We then use deep neural networks to output basic prediction and add proportional outputs of Kalman filter. Figure \ref{fig:results_two_three_step} shows that when FL-GCN is better than Kalman filter, there still exist some scenarios where the prediction errors in Kalman filter are less than those in deep neural networks, which indicates that Kalman filter can offset some worse predictions in FL-GCN. Combining both methods can increase prediction robustness to improve long-term performance.

The mixing parameter is a key factor in determining the final outputs. Figure \ref{fig:rmse_rmsn_ratio} shows that MAE, RMSE and RMSN would change with the ratio of deep neural networks under three prediction steps. The results indicate that prediction errors would firstly decrease as we increase the weight of neural networks. The curves have the lowest prediction errors when the ratio is 0.8. After that, prediction errors would increase as we add Kalman filter. The results show that deep neural networks play a major part in predicting O-D flows, and adding proportional outputs of Kalman filter could improve prediction performance.
%\clearpage
\begin{figure}[!ht]
  \centering
  \begin{subfigure}[b]{1.0\textwidth}
  \centering
  \includegraphics[width=0.63\textwidth, trim=50 110 100 160,clip]{figures//MAE.pdf}
  \caption{MAE performance}
  \end{subfigure}
  \hfill
  
  \begin{subfigure}[b]{1.0\textwidth}
  \centering
  \includegraphics[width=0.63\textwidth, trim=50 110 100 160,clip]{figures//RMSE.pdf}
  \caption{RMSE performance}
  \end{subfigure}
  \hfill
  
  \begin{subfigure}[b]{1.0\textwidth}
  \centering
  \includegraphics[width=0.63\textwidth, trim=50 110 100 160,clip]{figures//RMSN.pdf}
  \caption{RMSN performance}
  \end{subfigure}
  
  \caption{MAE, RMSE and RMSN with ratio of neural networks.} \label{fig:rmse_rmsn_ratio}
\end{figure}

\subsection{Interpretation of Graph Neural Networks}
In this section, we visualize and analyze the weights in converged deep neural networks \cite{zeiler2014visualizing, yosinski2015understanding}. In Equation \eqref{Equation: FL-GCN-CNN}, $\mathbf{w}_4$ denotes the weight in line graph convolution networks, and $\mathbf{w}_5$ represents the weight in historical O-D flows. We visualize the converged weights to show the effect of link flows and historical O-D flows. Figure \ref{fig:weight_his_OD} denotes the weight of historical O-D flows, and Figure \ref{fig:weight_link} shows the weight of link graph outputs. The results in the heat map show that historical weight $\mathbf{w}_5$ is larger than link weight $\mathbf{w}_4$, and the pattern is more significant in the diagonal direction, which indicates that historical O-D flows have greater impact than link flows on the final prediction.

\begin{figure}[!ht]
  \centering
  \begin{subfigure}[b]{1.0\textwidth}
  \centering
  \includegraphics[width=0.63\textwidth, trim=90 120 170 170,clip]{figures//his_od_weight.pdf}
  \caption{Historical O-D weight}
  \label{fig:weight_his_OD}
  \end{subfigure}
  \hfill
  
  \begin{subfigure}[b]{1.0\textwidth}
  \centering
  %\subfigure[Link flow weight]
  \includegraphics[width=0.63\textwidth, trim=90 120 170 170,clip]{figures//link_weight.pdf}
  \caption{Link flow weight}
  \label{fig:weight_link}
  \end{subfigure}
  
  \caption{Converged weights in convolutional neural networks  and graph neural networks.} \label{fig:weight}
\end{figure}

In Figure \ref{fig:results_two_three_step}, we can see that both FL-GCN and Kalman filter are inferred based on historical O-D flows and updated by link flows. FL-GCN incorporates historical O-D flows into deep neural networks, and utilizes CNN to recognize spatial correlations among O-D pairs. The prediction of Kalman filter is based on deviation from historical O-D flows, which also emphasizes the effect of historical O-D flows.
